Hierarchical Optimization for Whole-Body Control of Wheeled Inverted Pendulum Humanoids

In this paper, we present a whole-body control framework for Wheeled Inverted Pendulum (WIP) Humanoids. WIP Humanoids are redundant manipulators dynamically balancing themselves on wheels. Characterized by several degrees of freedom, they have the ability to perform several tasks simultaneously, such as balancing, maintaining a body pose, controlling the gaze, lifting a load or maintaining end-effector configuration in operation space. The problem of whole-body control is to enable simultaneous performance of these tasks with optimal participation of all degrees of freedom at specified priorities for each objective. The control also has to obey constraint of angle and torque limits on each joint. The proposed approach is hierarchical with a low level controller for body joints manipulation and a high-level controller that defines center of mass (CoM) targets for the low-level controller to control zero dynamics of the system driving the wheels. The low-level controller plans for shorter horizons while considering more complete dynamics of the system, while the high-level controller plans for longer horizon based on an approximate model of the robot for computational efficiency.

==> section2.tex <==
\section{Related Work} \label{sec:rel}



%\subsection{Whole-Body Control of Humanoids}
%Full body control of humanoids has attracted a lot of research interest recently. The approaches proposed are generally grounded in the broad framework of \cite{khatib1987unified}. This framework was initially introduced for unconstrained fully-actuated serial robots with stationary platforms. It allows the specification of tasks in workspace coordinates directly, and the controller solves for the required joint trajectories autonomously. Tasks are specified as cartesian positions/orientation or forces/torques and thus have six or less dimensions. For redundant systems, \ie that have more degrees of freedom (DOFs) than individual task dimensions, the framework allows for multiple lower-dimensional tasks to be simultaneously performed. Convex optimization can be utilized within this framework to handle constraints and optimize costs.
%
%This framework is extended for control of walking humanoids in \cite{sentis2006whole,sentis2010compliant}. It is a hierarchical approach where several priorities are defined such that each lower-priority task is projected in the combined null-space of tasks with priorities higher to it. Constraints and objectives are handled using virtual linkages. 
%
%Other hierarchical approaches \cite{de2010feature,escande2014hierarchical,herzog2014balancing,hutter2013hybrid,hutter2014quadrupedal,saab2013dynamic,wensing2013generation} explore the formulation of objectives and constraints as quadratic programs. Inverse dynamics (ID) approaches use system dynamics as one of the constraints when solving for target joint accelerations and torques. \cite{escande2014hierarchical} propose a generic solution to hierarchical quadratic programs that enforces equality and inequality constraints at all hierarchies, and is significantly faster than previous methods. 
%
%As opposed to hierarchical approaches that have hard priorities, \cite{feng2016online} prefer using weighted cost terms to specify preferences among the objectives. The compromise on precision it leads to is a trade-off to avoid the problem of ill-conditioned matrix inversions prevalent in hierarchical null-space approaches. They directly optimize a quadratic cost in terms of state acceleration, torques and contact forces using the full robot model. 
%
%Using inverse kinematics (IK) for tracking joint positions is also popular for controlling humanoid robots. A damped least squares method is used by \cite{nakamura1986inverse,wampler1986manipulator}. Using a similar approach, \cite{mistry2008inverse} compute the generalized velocity by inverting a matrix composed of end effector and contact constraint Jacobian. Computing only the generalized speeds $\dot{q}_{ik}$ and then integrating it to compute the corresponding positions $q_{ik}$ converges to local minima, but it produces continuous results reactive to online changes in the desired motions since optimization is performed at every time step.
%
%The framework we develop for WIP humanoid control is able to leverage this existing body of literature. We show this by isolating the manipulator/body dynamics from wheel dynamics. We present a detailed adaptation of the approach by \cite{sentis2006whole} into this framework, but other approaches can also be easily adapted.
%

%\subsection{Control of Wheeled Inverted Pendulum Systems}

%Wheeled Inverted Pendulum systems have been subjected to various control techniques including linear techniques implemented on the linearized model \cite{grasser2002joe,li2007mechanical,coelho2008development,huang2010development}, partial feedback linearization \cite{pathak2005velocity}, energy-shaping \cite{angeli2001almost}, fuzzy logic based control \cite{marzi2005multi,qingcheng2014fuzzy}, neural-network based control \cite{ren2008motion,jung2008control,tsai2010adaptive, wu2011ts}, hybrid controllers that switch between multiple controllers in different modes \cite{wu2011design,prasad2011optimal,fukushima2015sliding} and evolutionary algorithms for optimizing controllers \cite{ahmad2009genetic,goher2009ga,goher2010genetic} among many others. 

%Most techniques in this body of work consider the problem of controlling a one-link wheeled inverted pendulum model where the wheel torque is the primary control input controlling both the forward motion of the wheels and the balance of the inverted pendulum. Several joint torques present in the WIP humanoid body make for many control inputs in our case. And so, balancing the system purely using wheel-torque is neither necessary nor preferable. The entire upper body should participate in carrying out body balance as well as locomotion. This type of formulation is considered only by \cite{sasaki2008pushing,murakami2009motion,acar2011multi} and will be critically analyzed in the next subsection. But it is worth noting here that we control the wheel motion indirectly by controlling the zero dynamics that result from upper body control. We propose to do this  by precalculating an optimal control trajectory for upper body motions that minimize a tracking error for forward motion of the wheels. This allows the whole body to participate in controlling the center of mass as well as locomotion. The need to generate such a trajectory arises from the specific approach we take and therefore we rely on a novel controller based on differential dynamic programming (DDP) \Evangelos{Add a reference here}, a technique suitable for finding globally optimal trajectories for nonlinear systems and can potentially be extended to incorporate adaptive control to deal with modeling errors.

%\subsection{Whole-Body Control of Wheeled Inverted Pendulum Humanoids}
The specific problem of whole body control of WIP humanoids is addressed by Toshiyuki \etal \cite{sasaki2008pushing,murakami2009motion,acar2011multi}. The system under consideration in their work has a passive base joint. This means that the reaction torque due to wheel motors does not directly control the \textit{base link}---a term we use to identify the first link of the body attached to the wheels. They use null-space control, at the kinematic level, on only the actuated DOFs to find their reference accelerations for joint-level controllers. The passive joint is indirectly stabilized to always remain at a fixed position. In \cite{sasaki2008pushing}, only the wheels are stabilizing the passive joint by considering a simplified dynamic model of the system---a two-link WIP with first link representing the original passive joint and second representing the manipulator on top of it as a rigid body of an equivalent center of mass. In \cite{acar2011multi}, all active joints participate in this stabilization. In 
this work, they also propose a prioritization scheme such that lower-priority tasks are projected in the null-space of the jacobians of higher-priority ones. They perform three tasks, in the following order of priority: passive joint stabilization, end-effector positioning and center of mass control. The goal position of end-effector is in workspace coordinates in an inertial frame fixed on the ground, and their controller naturally generates locomotion trajectory if the goal location is not within immediate reach of the robot.

The problem of whole-body control of WIP humanoids with an active base joint however has not been addressed in the existing body of literature. In this case, the base joint is directly actuated by the reaction torque of the wheel motors. This happens when the wheel motors are mounted directly on the base link. This class of WIP systems are easier to build mechanically but pose a more challenging control problem due to the dynamics of the base link and the wheels being coupled by the wheel torque, in addition to the usual inertial coupling normally experienced by robotic systems. Most of the literature on WIP systems focuses on the first class of under-actuation (\ie passive base joint), which is mechanically more complex to build but offers a relatively easier control as the additional actuator torque coupling is not present. This fact is also noted by \cite{guo2014design}.

As we consider active base joint in this work, our approach fundamentally differs from Toshiyuki \etal \cite{acar2011multi} as their strategy treats the motion of the passive joint as the zero dynamics they indirectly control through actuated joint motions. Also, the base link in the structure they consider is a ``platform'' on top of which the fully actuated structure is mounted. They restrain this platform to stay at a fixed angular position. In general however, this is not necessary, as restricting the base link hinders its participation with other joints in performing the desired control tasks. The system we consider treats the base link as part of the manipulator/body performing the task, and the zero dynamics of the system are then derived that result from that control. The tasks for upper body are specified in a local frame of reference, which is fixed on the base such that it is stationary with respect to the upper body but moves with robot locomotion. Wheel motion is then controlled indirectly by finding optimal trajectories of body links to 
affect the zero dynamics to achieve that end. This strategy, as we will see, can easily accommodate the application of wide range of techniques offered by existing literature on redundant manipulators fixed on stationary platforms, once the issues that result from the wheel torque coupling are resolved. Robot locomotion is then treated as a higher-level task planned according to the desired workspace objectives.

Also, we demonstrate the application of inverse dynamics based approaches on WIP systems, as opposed to purely kinematics based approach proposed by Toshiyuki \etal Approaches based on inverse dynamics offer robustness to disturbances such as external force changes and result in compliant systems. However, only using inverse dynamics can perform poorly due to inevitable modeling errors generally unavoidable on real systems. So for implementation it is still important to generate kinematic targets for accurate motion.
